Decentralized Detection with Signaling

We consider a sequential problem in decentralized detection. Two observers can make repeated noisy observations of a binary hypothesis on the state of the environment. At any time, any of the two observers can stop and send a final message to the other observer or it may continue to take more measurements. After an observer has sent its final message, it stops operating. The other observer is then faced with a different stopping problem. At each time instant, it can decide either to stop and declare a final decision on the hypothesis or take another measurement. At each time, the system incurs an operating cost depending on the number of observers that are active at that time. A terminal cost that measures the accuracy of the final decision is incurred at the end. We show that, unlike in other sequential detection problems, stopping rules characterized by two thresholds on an observer's posterior belief no longer guarantee optimality in this problem. Thus the potential for signaling among observers alters the nature of optimal policies. We obtain a new parametric characterization of optimal policies for this problem.

==> Qualitative_properties.tex <==
\section{Qualitative Properties of Optimal Policies for O1} \label{sec:QP1}

\subsection{Information state for O1}
     Consider Problem P2 first. We first derive an information state for O1. For that purpose, we define:
     \begin{equation}
      \pi^1_t(Y^1_{1:t}) := P(H=0|Y^1_{1:t})
     \end{equation}
    The probability \(\pi^1_t\) is observer 1's belief on the hypothesis based on its sequence of observations till time \(t\). (For \(t=0\), we have \(\pi^1_0 = p_0\)). The following result provides a characterization of O1's optimal policy.
\begin{theorem}
  For Problem P2, with a fixed policy \(\Gamma^2\) of O2, there is an optimal policy for O1 of the form:
  \begin{equation} \label{eq:Qp1}
  Z^1_t = \gamma^1_{t}(\pi^{1}_{t})
  \end{equation}
  for \(t=1,2,...,T^1\).
  In particular, if globally optimal policies \(\Gamma^{1,*},\Gamma^{2,*}\) exist, then \(\Gamma^{1,*}\) can be assumed to be of the from in (\ref{eq:Qp1}) without loss of optimality. Moreover, for a fixed \(\Gamma^2\), the optimal policy of O1 can be determined by the following dynamic program:
  \begin{align}
    &V_{T^1}(\pi) := min \{ \nonumber \\ &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{T^1}=\pi,Z^1_{1:T^1-1}=b,Z^1_{T^1}=0],  \nonumber \\
                         &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{T^1}=\pi,Z^1_{1:T^1-1}=b,Z^1_{T^1}=1]  \}
 \end{align}   
 and for \(k=(T^1-1),...,2,1\),
 \begin{align}
  &V_{k}(\pi) := min\{ \nonumber \\ &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{k}=\pi,Z^1_{1:k-1}=b,Z^1_{k}=0], \nonumber \\
                          &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{k}=\pi,Z^1_{1:k-1}=b,Z^1_{k}=1], \nonumber \\
                          &c^1 + E^{\Gamma^2}[V_{k+1}(\pi^1_{k+1})|\pi^1_{k}=\pi,Z^1_{1:k}=b]                               \}
 \end{align}
 where the superscript \(\Gamma^2\) in the expectation denotes that the expectation is defined for a fixed choice of \(\Gamma^2\). (\(Z^1_{1:T^1-1}=b\) denotes a sequence of \(T^1-1\) blank messages.)
\end{theorem} 
\begin{IEEEproof}[Sketch of the Proof]
  Fix an arbitrary policy \(\Gamma^2 = (\gamma^2_1,\gamma^2_2,...,\gamma^2_{T2})\) for O2. It can be shown that if O1 has not sent its final message by time \(T^1-1\), the expected future cost for O1 at time \(T^1\) is one of the two terms in the minimization in \(V_{T^1}\) evaluated at \(\pi^1_{T^1}(y^1_{1:T^1})\). Thus, \(V_{T^1}\) evaluated at \(\pi^1_{T^1}(y^1_{1:T^1})\) provides a lower bound on the expected future cost at time \(T^1\). Following backward induction, it can be established that \(V_k(\pi^1_k(y^1_{1:k}))\) is a lower bound on the expected future cost if O1 has not sent a final message till time \(k-1\). (See [8] for details.) A policy \(\gamma^{*}\) that always selects the minimizing option in the definition of \(V_k\) for each \(\pi\) will achieve the lower bounds \(V_k\) on expected future cost with equality for all \(k\). This implies that \(\gamma^{*}\) achieves the lower bound on total cost for any policy. Hence, it is  optimal. Thus, an optimal policy is given by selecting the minimizing option in the definition of \(V_k\), \(k=1,2,...,T^1,\) at each \(\pi\). In other words, there is an optimal policy of the form:
 \[Z^1_t = \gamma^{*}_{t}(\pi^{1}_{t})\] 
  % Hence, there is a globally optimal policy of O1 of the form %in (\ref{eq:Qp1}). 
\end{IEEEproof}    
%\hspace{5pt} \emph{Corollary:} There is a globally optimal policy for O1 of the form in (\ref{eq:Qp1}) in Problem P1 also. 
\hspace{5pt} \emph{Corollary:} Theorem 1 holds for O1 in Problem P1 also.
\begin{proof}[Sketch of the Proof]
	In the proof of Theorem 1, we fixed \(\Gamma^2\) to any arbitrary choice. In particular, consider any policy of O2 that waits till it gets a final decision from O1. After it receives the final message from O1 at time \(\tau^1\), it uses only observations made after \(\tau^1\) to make a decision. This class of policies is essentially the policies available to O2 in problem P1. Since the optimal structure of O1's policy as given in (\ref{eq:Qp1}) holds for any choice of \(\Gamma^2\), it also holds for all possible policies of O2 in problem P1. See [8] for details. 
\end{proof} 
%\begin{IEEEproof}
%See [8].
%\end{IEEEproof}

%\begin{proof}
%	In the proof of Theorem 1, we fixed \(\Gamma^2\) to any arbitrary choice. In particular, consider any policy of O2 that waits till it gets a %final decision from O1. After it receives the final message from O1 at time \(\tau^1\), it uses only observations made after \(\tau^1\) to make %a decision. This class of policies is essentially the policies available to O2 in problem P1. Since the optimal structure of O1's policy as %given in (\ref{eq:Qp1}) holds for any choice of \(\Gamma^2\), it also holds for all possible policies of O2 in problem P1.  
%\end{proof}

   The result of Theorem 1 can be intuitively explained as follows. At any time \(t\), if the observer 1 has not already sent its final message, it has to choose between three choices of action - send \(0,1\) or \(b\). In order to evaluate the expected cost of sending a \(0\) or \(1\), O1 needs a belief on the state of the environment, that is, a belief on \(H\) and a belief on the information available to O2. Since O1 has not yet sent a final message, the information at O2 consists of \(Z^1_{1:t-1} = b_{1:t-1}\), what O1 decides to send as \(Z^1_t\) and the observations that O2 has made or may make in the future. Thus O1 needs to form a belief on \(Y^2_{1:T^2}\), since the rest of O2's information it already knows. Now because of conditional independence of observations at the two observers, it is sufficient to form a belief on \(H\)  to know the probabilities of \(Y^2_{1:T^2}\). Similarly, to evaluate the cost of sending a \(b\), O1 needs to form a belief on O2's information and what information O1 may obtain by future measurements-\(Y^1_{t+1:T^1}\). Once again, conditional independence of observations made at different times given \(H\) implies a belief on \(H\) is sufficient to evaluate the cost of this action as well. These arguments indicate that the decisions at O1 should be made based only on its belief on \(H\), that is, \(\pi^1_t\).  
\subsection{Classical Threshold Rules Are Not Optimal}
      In sequential detection problem with a single observer [7], it is well known that an optimal policy is a function of the observer's belief \(\pi_t\) and is described by two thresholds at each time \(t\). That is the decision at time \(t\), \(Z_t\) is given as:
      \[ Z_t = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi_t \leq \alpha_t$} \\
               N & \mbox{if $\alpha_t<\pi_t < \beta_t$} \\
               0 & \mbox{if $\pi_t \geq \beta_t$}
               \end{array}
               \right. \]
     where \(N\) denotes a decision to continue taking measurement and \(\alpha_t \leq \beta_t\) are real numbers in \([0,1]\).
 A similar two-threshold structure of optimal policies was also established for the decentralized Wald problem in [2]. We will show by means of two counterexamples that such a structure is not necessarily optimal for observer 1 in Problem P1. 
 \par
 \emph{Example 1} 
 \par
 Consider the following instance of Problem P1. We have equal prior on \(H\), that is \(P(H=0)=P(H=1)=1/2\). O1 has a time horizon of \(T^1=2\). Its observation space is \(\mathcal{Y}^1 = \{1,2,3\}\). The observations at time \(t=1\) follow the following conditional probabilities:
 \[ \begin{array}{lclc}
Observation & 1 & 2 & 3 \\
P(.|H=0)    & 0 & p & (1-p) \\
P(.|H=1)    & (1-p) & p & 0 
\end{array}\]
and at time \(t=2\) follow the following conditional probabilities:
\[ \begin{array}{lclc}
Observation & 1 & 2 & 3 \\
P(.|H=0)    & 0 & q & (1-q) \\
P(.|H=1)    & (1-q) & q & 0 
\end{array}\]
where \(p,q \in [0,1]\).
Observe that O1's belief on \(\{H=0\}\) (that is, \(\pi^1\)), only takes 3 possible values - \(0,1\) and \(1/2\) after any number of measurements.
O1 has to send a final message - \(0\) or \(1\) - to O2 by time \(t=2\). If O1 delays sending its final message to time \(t=2\), an additional cost \(c^1\) is incurred. After receiving a message from O1, observer 2 can either declare a decision on the hypothesis or take at most 1 more measurement of its own, that is, we have \(T^2 =1\). The measurements of O2 are assumed to be noiseless, so when O2 takes a measurement it knows exactly the value of \(H\). However, the measurement comes at a cost of \(c^2\). We assume that \(J(U,H) =0\) if \(U=H\), and in the case of  a mistake \((U \neq H)\), we assume that the cost is sufficiently high so that unless O2 is certain from O1's messages what the true hypothesis is, it will prefer taking a measurement at a cost \(c^2\) than making a guess. 
  At \(p=0.6\), \(c^2 > 3c^1\), it can be easily verified that the best threshold rule for observer 1 is described as follows:
  \begin{itemize}
  \item At \(t=1\), \[ Z_t = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^1_t = 0$} \\
               b & \mbox{if $\pi^1_t = 1/2$} \\
               0 & \mbox{if $\pi^1_t = 1$}
               \end{array}
               \right. \]
  \item At \(t=2\), \[ Z_t = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^1_t = 0$} \\
               0 & \mbox{if $\pi^1_t \geq 1/2$}               
               \end{array}
               \right. \]
  \end{itemize}
  
  %\begin{itemize}
  %\item At \(t=1\), send \(0\) if \(\pi^1 = 1\), send \(1\) if \(\pi^1 =0\) and send \(b\) if \(\pi^1 = 1/2\).
  %\item At \(t=2\), send \(0\) if \(\pi^1\) is either \(1\) or \(1/2\), send \(1\) otherwise.
  %\end{itemize}
  If observer 2 receives \(0\) or \(1\) at time \(t=1\), it declares the received message as the final decision on the hypothesis, otherwise it waits for a final message from O1. At \(t=2\), if O2 receives \(1\), it declares \(1\) as the final decision, otherwise it takes a measurement. Then the expected cost of this policy is given as: \( pc^1 + p(1+q)c^2/2\) (since the system incurs a cost \(c^1\) with probability \(p\) and a cost \(c^2\) with probability \(p/2 + pq/2\)).
  \par
  Now consider the following non-threshold policy for observer 1.
  \begin{itemize}
  \item At \(t=1\), \[ Z_t = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^1_t = 0$} \\
               0 & \mbox{if $\pi^1_t = 1/2$} \\
               b & \mbox{if $\pi^1_t = 1$}
               \end{array}
               \right. \]
  \item At \(t=2\), \[ Z_t = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^1_t = 0$} \\
               0 & \mbox{if $\pi^1_t \geq 1/2$}               
               \end{array}
               \right. \]
  \end{itemize} 
  %\begin{itemize}
  %\item At \(t=1\), send \(0\) if \(\pi^1 = 1/2\), send \(b\) otherwise.
  %\item At \(t=2\), send \(0\) if \(\pi^1\) is either \(1\) or \(1/2\), send \(1\) otherwise.
  %\end{itemize}
  If observer 2 receives \(0\) at time \(t=1\), it takes a measurement and incurs a cost \(c^2\). If O2 receives a \(1\) at \(t=1\), it declares \(1\) as the final decision. If O2 receives a \(b\) at time \(t=1\), it waits for the final message at \(t=2\) and then declares the received message as its final decision on the hypothesis.  Then the expected cost of this policy is given as: \( pc^2 + (1-p)c^1/2\) (since the system incurs a cost \(c^2\) with probability \(p\) and a cost \(c^1\) with probability \((1-p)/2\)). It is now easily seen that at \(p=0.6\) and \(c^2>6c^1\), if we choose \(q > 1-\frac{4c^1}{3c^2}\), the non-threshold policy outperforms the best threshold policy.

 \emph{Discussion of the Example:} The principle behind a threshold rule is to stop and send a message if O1 is certain, otherwise postpone the decision and take another measurement. The additional cost of delay is justified by the likelihood of getting a good measurement in the next time instant. In our example, if O1 gets the observations \(1\) or \(3\) at \(t=1\) and is able to convey to O2 that it is certain about the true hypothesis and what this hypothesis is, then it prevents O2 from taking a measurement thus saving a cost \(c^2\). The threshold rule achieves this objective by sending \(0\) for observation \(3\) and \(1\) for observation \(1\). However, in the case when O1 gets measurement \(2\), it decides to wait for the next observation. By choosing \(q\) sufficiently high, the likelihood of getting a good measurement at \(t=2\) can be made very low. In this case, the cost of delaying a decision \((c^1)\) begins outweighing the expected payoff from a new measurement. The non-threshold rule essentially tries to correct this drawback. If at time \(t=1\), O1 gets measurement \(2\), it stops and sends \(0\) to O2. At O2, this is interpreted as a message to go and take measurement of its own. Note that the non-threshold rule still ensures that whenever O1 is certain about \(H\), it is able to send enough information to O2 to prevent it from taking a measurement.  
 %O1's policy above can be explained as follows. In case, O1's observation is sufficient to know what the true \(H\) is (that is in case of observation 1 and 4), O1 should be able to convey to O2 the true value of \(H\) \emph{and} the fact that it is certain about the true value. This will allow O2 to make a decision without making its own measurement, thus saving on the term \(c^2\). On the other hand, in case O1 is not sure of the true hypothesis, it should be able to convey to O2 -as quickly as possible- that this is the case. Any delay in conveying that O1 is not sure of \(H\) incurs a penalty \(c^1\) (as we said before, \(c^1\) could model various kind of costs including that the system has to pay in say keeping the receiving antennas of O2 on while its expecting a message from O1). A good threshold rule could be to send a \(0\) or \(1\) at \(t=1\) depending on whether the observation was \(4\) or \(1\) and blank otherwise. This will certainly achieve the first objective, that is, to convey that O1 knows the value of \(H\) for sure and that this value is the transmitted symbol. However, with a probability \(p\), O1 will delay conveying the information that it was not sure of \(H\), thus incurring a penalty \(c^1\). When \(p\) is sufficiently large, this penalty term dominates.  The non-threshold rule shown above minimizes this term-by sending a \(0\) or \(1\) when O1 is not sure of \(H\). Then, if O2 receives \(b\) from O1, it already knows that O1 is sure of \(H\). It waits for a final message from O1 that informs it of the true \(H\) -the system incurs the corresponding penalty of \(c^1\), but now only for an event of probability \(1-p\). 
 \par
 \emph{Example 2}\\
  As before, we have an instance of Problem P1 where Observer 1 has a time horizon of \(T^1=2\). Its observations at \(t=1\) are given by the following conditional probabilities.  
\[ \begin{array}{lcccc}
Observation & 1 & 2 & 3 & 4 \\
P(.|H=0)    & 0 & p/3 & 2p/3 & (1-p) \\
P(.|H=1)    & (1-p) & 2p/3 & p/3 & 0 
\end{array}\]
O1's observations at time \(t=2\) are just noise and give no new information. Note that the observations are indexed in order of the posterior belief \(\pi^1\) they generate, that is, \(P(H=0|Observation 1) < P(H=0|Observation 2)\) and so on. Observer 2 can make a noiseless measurement at a cost of \(c^2\). Observer 2's cost of making a wrong decision is chosen sufficiently high so that unless it is certain from O1's message what the true hypothesis is, O2 will prefer taking a measurement at a cost \(c^2\) than making a guess.
It can be shown that for equal prior (\( p_0 =1/2\)), \(c^2>2c^1\) and \(1/2<p<1\), a non-threshold rule for O1 (given below) performs better than any threshold policy. 
\begin{itemize}
\item At \(t=1\), send \(0\) if observation 2 occurs and \(1\) if observation 3 occurs. Send a blank otherwise otherwise.
\item At \(t=2\), send \(1\) if the posterior belief on \((H=0)\) is less than \(1/2\) and \(0\) otherwise.
\end{itemize} 

 \subsection{Parametric Characterization of Optimal Policies}
   An important advantage of the threshold rules in the case of the centralized or the decentralized Wald problem is that it modifies the problem of finding the globally optimal policies from a sequential functional optimization problem to a sequential parametric optimization problem. Even though we have established that a classical threshold rule does not hold for our problem, it is still possible to get a finite parametric characterization of an optimal policy for observer 1. Such a parametric characterization provides significant computational advantage in finding optimal policies, for example by reducing the search space for an optimal policy.         \par
 In Theorem 1, we have established  that for an arbitrarily fixed choice of O2's policy, the optimal policy for O1 can be determined by backward induction using the functions \(V_k(\pi), k=T^1,...,2,1\). We will call \(V_k\) the value function at time \(k\).
 We have the following lemma.
 \begin{lemma}
  With a fixed (but arbitrary) choice of \(\Gamma^2\), the value function at \(T^1\) can be expressed as:
  \begin{equation}
  V_{T^1}(\pi) := min\{ L^{0}_{T^1}(\pi), L^{1}_{T^1}(\pi)\}
  \end{equation}
  where \(L^{0}_{T^1}\) and \(L^{1}_{T^1}\) are affine functions of \(\pi\) that depend on the choice of O2's policy \(\Gamma^2\).
  Also, the value function at time \(k\) can be expressed as:
  \begin{equation}\label{eq:PFlemma1}
  V_{k}(\pi) := min\{ L^{0}_k(\pi), L^{1}_k(\pi), G_k(\pi)\}
  \end{equation}
  where \(L^{0}_{k}\) and \(L^{1}_{k}\) are affine functions of \(\pi\) and \(G_k\) is a concave function of \(\pi\) that depend on the choice of \(\Gamma^2\).
 \end{lemma}
 \begin{IEEEproof}
 See Appendix A.
\end{IEEEproof}
 
 \begin{theorem}
  For any fixed policy \(\Gamma^2\) of O2,  an optimal policy for O1 can be characterized by \emph{at most 4 thresholds}. In particular, an optimal policy for O1 is of the form:
   \[ Z^1_{T^1} = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^1_{T^1} \leq \alpha_{T^1}$} \\
               0 & \mbox{if $\pi^1_{T^1} > \alpha_{T^1}$ }
               \end{array}
               \right. \]
               where \(0 \leq \alpha_{T^1} \leq 1\)  and for \(k=1,2,..,T^1-1\),
         \[ Z^1_k = \left \{ \begin{array}{ll}
               b & \mbox{if $\pi^1_k < \alpha_k$}  \\
               1 & \mbox{if $\alpha_k \leq \pi^1_k \leq \beta_k$} \\
               b & \mbox{if $\beta_k<\pi^1_k < \delta_k$} \\
               0 & \mbox{if $\delta_k \leq \pi^1_k \leq \theta_k$} \\
               b & \mbox{if $\pi^1_k > \theta_k$}
               \end{array}
               \right. \]  
               where \(0 \leq \alpha_k \leq \beta_k \leq \delta_k \leq \theta_k \leq 1\). 
\end{theorem}
\begin{IEEEproof}
Theorem 2 is an immediate consequence of Lemma 1, since taking minimum of straight lines and concave functions can partition the interval \( [0,1]\) into at most  five regions. The thresholds above essentially signify the boundaries of these regions. 
\end{IEEEproof}
 It is of course possible that in specific cases, some of these five regions are absent which would correspond to some of the above thresholds having the same value. For example, in the non-threshold rule given in the counterexample earlier, the rule at \(t=1\) corresponds to having \(\alpha=0\) and 
\(\beta=\delta\) which results in a 3-interval partition of \([0,1]\) corresponding the rule given there.


==> Qualitative_properties_v2.tex <==
\section{Qualitative Properties of Optimal Policies for O1} \label{sec:QP1}

\subsection{Information state for O1}
     Consider Problem P2 first. We first derive an information state for O1. For that purpose, we define:
     \begin{equation}
      \pi^1_t(Y^1_{1:t}) := P(H=0|Y^1_{1:t})
     \end{equation}
    The probability \(\pi^1_t\) is observer 1's belief on the hypothesis based on its sequence of observations till time \(t\). (For \(t=0\), we have \(\pi^1_0 = p_0\)). The following result provides a characterization of O1's optimal policy.
\begin{theorem}
  For Problem P2, with a fixed policy \(\Gamma^2\) of O2, there is an optimal policy for O1 of the form:
  \begin{equation} \label{eq:Qp1}
  Z^1_t = \gamma^1_{t}(\pi^{1}_{t})
  \end{equation}
  for \(t=1,2,...,T^1\).
  In particular, if globally optimal policies \(\Gamma^{1,*},\Gamma^{2,*}\) exist, then \(\Gamma^{1,*}\) can be assumed to be of the from in (\ref{eq:Qp1}) without loss of optimality. Moreover, for a fixed \(\Gamma^2\), the optimal policy of O1 can be determined by the following dynamic program:
  \begin{align}
    &V_{T^1}(\pi) := min \{ \nonumber \\ &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{T^1}=\pi,Z^1_{1:T^1-1}=b,Z^1_{T^1}=0],  \nonumber \\
                         &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{T^1}=\pi,Z^1_{1:T^1-1}=b,Z^1_{T^1}=1]  \}
 \end{align}   
 and for \(k=(T^1-1),...,2,1\),
 \begin{align}
  &V_{k}(\pi) := min\{ \nonumber \\ &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{k}=\pi,Z^1_{1:k-1}=b,Z^1_{k}=0], \nonumber \\
                          &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{k}=\pi,Z^1_{1:k-1}=b,Z^1_{k}=1], \nonumber \\
                          &c^1 + E^{\Gamma^2}[V_{k+1}(\pi^1_{k+1})|\pi^1_{k}=\pi,Z^1_{1:k}=b]                               \}
 \end{align}
 where the superscript \(\Gamma^2\) in the expectation denotes that the expectation is defined for a fixed choice of \(\Gamma^2\). (\(Z^1_{1:T^1-1}=b\) denotes a sequence of \(T^1-1\) blank messages.)
\end{theorem} 
\begin{IEEEproof}[Sketch of the Proof]
  Fix an arbitrary policy \(\Gamma^2 = (\gamma^2_1,\gamma^2_2,...,\gamma^2_{T2})\) for O2. It can be shown that if O1 has not sent its final message by time \(T^1-1\), the expected future cost for O1 at time \(T^1\) is one of the two terms in the minimization in \(V_{T^1}\) evaluated at \(\pi^1_{T^1}(y^1_{1:T^1})\). Thus, \(V_{T^1}\) evaluated at \(\pi^1_{T^1}(y^1_{1:T^1})\) provides a lower bound on the expected future cost at time \(T^1\). Following backward induction, it can be established that \(V_k(\pi^1_k(y^1_{1:k}))\) is a lower bound on the expected future cost if O1 has not sent a final message till time \(k-1\). (See [8] for details.) A policy \(\gamma^{*}\) that always selects the minimizing option in the definition of \(V_k\) for each \(\pi\) will achieve the lower bounds \(V_k\) on expected future cost with equality for all \(k\). This implies that \(\gamma^{*}\) achieves the lower bound on total cost for any policy. Hence, it is  optimal. Thus, an optimal policy is given by selecting the minimizing option in the definition of \(V_k\), \(k=1,2,...,T^1,\) at each \(\pi\). In other words, there is an optimal policy of the form:
 \[Z^1_t = \gamma^{*}_{t}(\pi^{1}_{t})\] 
  % Hence, there is a globally optimal policy of O1 of the form %in (\ref{eq:Qp1}). 
\end{IEEEproof}    
%\hspace{5pt} \emph{Corollary:} There is a globally optimal policy for O1 of the form in (\ref{eq:Qp1}) in Problem P1 also. 
\hspace{5pt} \emph{Corollary:} Theorem 1 holds for O1 in Problem P1 also.
\begin{proof}[Sketch of the Proof]
	In the proof of Theorem 1, we fixed \(\Gamma^2\) to any arbitrary choice. In particular, consider any policy of O2 that waits till it gets a final decision from O1. After it receives the final message from O1 at time \(\tau^1\), it uses only observations made after \(\tau^1\) to make a decision. This class of policies is essentially the policies available to O2 in problem P1. Since the optimal structure of O1's policy as given in (\ref{eq:Qp1}) holds for any choice of \(\Gamma^2\), it also holds for all possible policies of O2 in problem P1. See [8] for details. 
\end{proof} 
%\begin{IEEEproof}
%See [8].
%\end{IEEEproof}

%\begin{proof}
%	In the proof of Theorem 1, we fixed \(\Gamma^2\) to any arbitrary choice. In particular, consider any policy of O2 that waits till it gets a %final decision from O1. After it receives the final message from O1 at time \(\tau^1\), it uses only observations made after \(\tau^1\) to make %a decision. This class of policies is essentially the policies available to O2 in problem P1. Since the optimal structure of O1's policy as %given in (\ref{eq:Qp1}) holds for any choice of \(\Gamma^2\), it also holds for all possible policies of O2 in problem P1.  
%\end{proof}

   The result of Theorem 1 can be intuitively explained as follows. At any time \(t\), if the observer 1 has not already sent its final message, it has to choose between three choices of action - send \(0,1\) or \(b\). In order to evaluate the expected cost of sending a \(0\) or \(1\), O1 needs a belief on the state of the environment, that is, a belief on \(H\) and a belief on the information available to O2. Since O1 has not yet sent a final message, the information at O2 consists of \(Z^1_{1:t-1} = b_{1:t-1}\), what O1 decides to send as \(Z^1_t\) and the observations that O2 has made or may make in the future. Thus O1 needs to form a belief on \(Y^2_{1:T^2}\), since the rest of O2's information it already knows. Now because of conditional independence of observations at the two observers, it is sufficient to form a belief on \(H\)  to know the probabilities of \(Y^2_{1:T^2}\). Similarly, to evaluate the cost of sending a \(b\), O1 needs to form a belief on O2's information and what information O1 may obtain by future measurements-\(Y^1_{t+1:T^1}\). Once again, conditional independence of observations made at different times given \(H\) implies a belief on \(H\) is sufficient to evaluate the cost of this action as well. These arguments indicate that the decisions at O1 should be made based only on its belief on \(H\), that is, \(\pi^1_t\).  
\subsection{Classical Threshold Rules Are Not Optimal}
      In the sequential detection problem with a single observer [7], it is well known that an optimal policy is a function of the observer's belief \(\pi_t\) and is described by two thresholds at each time \(t\). That is the decision at time \(t\), \(Z_t\) is given as:
      \[ Z_t = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi_t \leq \alpha_t$} \\
               N & \mbox{if $\alpha_t<\pi_t < \beta_t$} \\
               0 & \mbox{if $\pi_t \geq \beta_t$}
               \end{array}
               \right. \]
     where \(N\) denotes a decision to continue taking measurement and \(\alpha_t \leq \beta_t\) are real numbers in \([0,1]\).
 A similar two-threshold structure of optimal policies was also established for the decentralized Wald problem in [2]. We will show by means of two counterexamples that such a structure is not necessarily optimal for observer 1 in Problem P1. 
 \par
 \emph{Example 1} 
 \par
 Consider the following instance of Problem P1. We have equal prior on \(H\), that is \(P(H=0)=P(H=1)=1/2\). O1 has a time horizon of \(T^1=2\). Its observation space is \(\mathcal{Y}^1 = \{1,2,3\}\). The observations at time \(t=1\) follow the following conditional probabilities:
 \[ \begin{array}{lclc}
Observation & 1 & 2 & 3 \\
P(.|H=0)    & 0 & p & (1-p) \\
P(.|H=1)    & (1-p) & p & 0 
\end{array}\]
and at time \(t=2\) follow the following conditional probabilities:
\[ \begin{array}{lclc}
Observation & 1 & 2 & 3 \\
P(.|H=0)    & 0 & q & (1-q) \\
P(.|H=1)    & (1-q) & q & 0 
\end{array}\]
where \(p,q \in [0,1]\).
Observe that O1's belief on \(\{H=0\}\) (that is, \(\pi^1\)), only takes 3 possible values - \(0,1\) and \(1/2\) after any number of measurements.
O1 has to send a final message - \(0\) or \(1\) - to O2 by time \(t=2\). If O1 delays sending its final message to time \(t=2\), an additional cost \(c^1\) is incurred. After receiving a message from O1, observer 2 can either declare a decision on the hypothesis or take at most 1 more measurement of its own, that is, we have \(T^2 =1\). The measurements of O2 are assumed to be noiseless, so when O2 takes a measurement it knows exactly the value of \(H\). However, the measurement comes at a cost of \(c^2\). We assume that \(J(U,H) =0\) if \(U=H\), and in the case of  a mistake \((U \neq H)\), we assume that the cost is sufficiently high so that unless O2 is certain from O1's messages what the true hypothesis is, it will prefer taking a measurement at a cost \(c^2\) than making a guess. 
  At \(p=0.6\), \(c^2 > 3c^1\), it can be easily verified that the best threshold rule for observer 1 is described as follows:
  \begin{itemize}
  \item At \(t=1\), send \(1\) if \(\pi^1_1 = 0\), send \(b\) if \(\pi^1_1 = 1/2\) and send \(0\) if \(\pi^1_1 = 1\).
  \item At \(t=2\), send \(1\) if \(\pi^1_2 = 0\), send \(0\) otherwise.
  \end{itemize}
  
  %\begin{itemize}
  %\item At \(t=1\), send \(0\) if \(\pi^1 = 1\), send \(1\) if \(\pi^1 =0\) and send \(b\) if \(\pi^1 = 1/2\).
  %\item At \(t=2\), send \(0\) if \(\pi^1\) is either \(1\) or \(1/2\), send \(1\) otherwise.
  %\end{itemize}
  If observer 2 receives \(0\) or \(1\) at time \(t=1\), it declares the received message as the final decision on the hypothesis, otherwise it waits for a final message from O1. At \(t=2\), if O2 receives \(1\), it declares \(1\) as the final decision, otherwise it takes a measurement. Then the expected cost of this policy is given as: \( pc^1 + p(1+q)c^2/2\) (since the system incurs a cost \(c^1\) with probability \(p\) and a cost \(c^2\) with probability \(p/2 + pq/2\)).
  \par
  Now consider the following non-threshold policy for observer 1,
  \begin{itemize}
  \item At \(t=1\), send \(1\) if \(\pi^1_1 = 0\), send \(0\) if \(\pi^1_1 = 1/2\) and send \(b\) if \(\pi^1_1 = 1\).
  \item At \(t=2\), send \(1\) if \(\pi^1_2 = 0\), send \(0\) otherwise.
  \end{itemize} 
  %\begin{itemize}
  %\item At \(t=1\), send \(0\) if \(\pi^1 = 1/2\), send \(b\) otherwise.
  %\item At \(t=2\), send \(0\) if \(\pi^1\) is either \(1\) or \(1/2\), send \(1\) otherwise.
  %\end{itemize}
  If observer 2 receives \(0\) at time \(t=1\), it takes a measurement and incurs a cost \(c^2\). If O2 receives a \(1\) at \(t=1\), it declares \(1\) as the final decision. If O2 receives a \(b\) at time \(t=1\), it waits for the final message at \(t=2\) and then declares the received message as its final decision on the hypothesis.  Then the expected cost of this policy is given as: \( pc^2 + (1-p)c^1/2\) (since the system incurs a cost \(c^2\) with probability \(p\) and a cost \(c^1\) with probability \((1-p)/2\)). It is now easily seen that at \(p=0.6\) and \(c^2>3c^1\), if we choose \(q > 1-\frac{4c^1}{3c^2}\), the non-threshold policy outperforms the best threshold policy.

 \emph{Discussion of the Example:} The principle behind a threshold rule is to stop and send a message if O1 is certain, otherwise postpone the decision and take another measurement. The additional cost of delay is justified by the likelihood of getting a good measurement in the next time instant. In our example, if O1 gets the observations \(1\) or \(3\) at \(t=1\) and is able to convey to O2 that it is certain about the true hypothesis and what this hypothesis is, then it prevents O2 from taking a measurement thus saving a cost \(c^2\). The threshold rule achieves this objective by sending \(0\) for observation \(3\) and \(1\) for observation \(1\). However, in the case when O1 gets measurement \(2\), it decides to wait for the next observation. By choosing \(q\) sufficiently high, the likelihood of getting a good measurement at \(t=2\) can be made very low. In this case, the cost of delaying a decision \((c^1)\) begins outweighing the expected payoff from a new measurement. The non-threshold rule essentially tries to correct this drawback. If at time \(t=1\), O1 gets measurement \(2\), it stops and sends \(0\) to O2. At O2, this is interpreted as a message to go and take measurement of its own. Note that the non-threshold rule still ensures that whenever O1 is certain about \(H\), it is able to send enough information to O2 to prevent it from taking a measurement.  
 %O1's policy above can be explained as follows. In case, O1's observation is sufficient to know what the true \(H\) is (that is in case of observation 1 and 4), O1 should be able to convey to O2 the true value of \(H\) \emph{and} the fact that it is certain about the true value. This will allow O2 to make a decision without making its own measurement, thus saving on the term \(c^2\). On the other hand, in case O1 is not sure of the true hypothesis, it should be able to convey to O2 -as quickly as possible- that this is the case. Any delay in conveying that O1 is not sure of \(H\) incurs a penalty \(c^1\) (as we said before, \(c^1\) could model various kind of costs including that the system has to pay in say keeping the receiving antennas of O2 on while its expecting a message from O1). A good threshold rule could be to send a \(0\) or \(1\) at \(t=1\) depending on whether the observation was \(4\) or \(1\) and blank otherwise. This will certainly achieve the first objective, that is, to convey that O1 knows the value of \(H\) for sure and that this value is the transmitted symbol. However, with a probability \(p\), O1 will delay conveying the information that it was not sure of \(H\), thus incurring a penalty \(c^1\). When \(p\) is sufficiently large, this penalty term dominates.  The non-threshold rule shown above minimizes this term-by sending a \(0\) or \(1\) when O1 is not sure of \(H\). Then, if O2 receives \(b\) from O1, it already knows that O1 is sure of \(H\). It waits for a final message from O1 that informs it of the true \(H\) -the system incurs the corresponding penalty of \(c^1\), but now only for an event of probability \(1-p\). 
 \par
 \emph{Example 2}\\
  Consider the same problem as in Example 1 but with O1's observations at \(t=1\) now given by the following conditional probabilities.  
\[ \begin{array}{lcccc}
Observation & 1 & 2 & 3 & 4 \\
P(.|H=0)    & 0 & p/3 & 2p/3 & (1-p) \\
P(.|H=1)    & (1-p) & 2p/3 & p/3 & 0 
\end{array}\]
O1's observations at time \(t=2\) are just noise and give no new information. Note that the observations are indexed in order of the posterior belief \(\pi^1\) they generate, that is, \(P(H=0|Observation 1) < P(H=0|Observation 2)\) and so on. 
It can be shown that for equal prior (\( p_0 =1/2\)), \(c^2>2c^1\) and \(1/2<p<1\), a non-threshold rule for O1 (given below) performs better than any threshold policy. 
\begin{itemize}
\item At \(t=1\), send \(0\) if observation 2 occurs and \(1\) if observation 3 occurs. Send a blank otherwise.
\item At \(t=2\), send \(1\) if \(\pi^1_2\) is less than \(1/2\) and \(0\) otherwise.
\end{itemize} 

 \subsection{Parametric Characterization of Optimal Policies}
   An important advantage of the threshold rules in the case of the centralized or the decentralized Wald problem is that it modifies the problem of finding the globally optimal policies from a sequential functional optimization problem to a sequential parametric optimization problem. Even though we have established that a classical threshold rule does not hold for our problem, it is still possible to get a finite parametric characterization of an optimal policy for observer 1. Such a parametric characterization provides significant computational advantage in finding optimal policies, for example by reducing the search space for an optimal policy.         \par
 In Theorem 1, we have established  that for an arbitrarily fixed choice of O2's policy, the optimal policy for O1 can be determined by backward induction using the functions \(V_k(\pi), k=T^1,...,2,1\). We will call \(V_k\) the value function at time \(k\).
 We have the following lemma.
 \begin{lemma}
  With a fixed (but arbitrary) choice of \(\Gamma^2\), the value function at \(T^1\) can be expressed as:
  \begin{equation}
  V_{T^1}(\pi) := min\{ L^{0}_{T^1}(\pi), L^{1}_{T^1}(\pi)\}
  \end{equation}
  where \(L^{0}_{T^1}\) and \(L^{1}_{T^1}\) are affine functions of \(\pi\) that depend on the choice of O2's policy \(\Gamma^2\).
  Also, the value function at time \(k\) can be expressed as:
  \begin{equation}\label{eq:PFlemma1}
  V_{k}(\pi) := min\{ L^{0}_k(\pi), L^{1}_k(\pi), G_k(\pi)\}
  \end{equation}
  where \(L^{0}_{k}\) and \(L^{1}_{k}\) are affine functions of \(\pi\) and \(G_k\) is a concave function of \(\pi\) that depend on the choice of \(\Gamma^2\).
 \end{lemma}
 \begin{IEEEproof}
 See Appendix A.
\end{IEEEproof}
 
 \begin{theorem}
  For any fixed policy \(\Gamma^2\) of O2,  an optimal policy for O1 can be characterized by \emph{at most 4 thresholds}. In particular, an optimal policy for O1 is of the form:
   \[ Z^1_{T^1} = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^1_{T^1} \leq \alpha_{T^1}$} \\
               0 & \mbox{if $\pi^1_{T^1} > \alpha_{T^1}$ }
               \end{array}
               \right. \]
               where \(0 \leq \alpha_{T^1} \leq 1\)  and for \(k=1,2,..,T^1-1\),
         \[ Z^1_k = \left \{ \begin{array}{ll}
               b & \mbox{if $\pi^1_k < \alpha_k$}  \\
               1 & \mbox{if $\alpha_k \leq \pi^1_k \leq \beta_k$} \\
               b & \mbox{if $\beta_k<\pi^1_k < \delta_k$} \\
               0 & \mbox{if $\delta_k \leq \pi^1_k \leq \theta_k$} \\
               b & \mbox{if $\pi^1_k > \theta_k$}
               \end{array}
               \right. \]  
               where \(0 \leq \alpha_k \leq \beta_k \leq \delta_k \leq \theta_k \leq 1\). 
\end{theorem}
\begin{IEEEproof}
Theorem 2 is an immediate consequence of Lemma 1, since taking minimum of straight lines and concave functions can partition the interval \( [0,1]\) into at most  five regions. The thresholds above essentially signify the boundaries of these regions. 
\end{IEEEproof}
 It is of course possible that in specific cases, some of these five regions are absent which would correspond to some of the above thresholds having the same value. For example, in the non-threshold rule given in the Example 1 earlier, the rule at \(t=1\) corresponds to having \(\alpha=0\) and 
\(\beta=\delta\) which results in a 3-interval partition of \([0,1]\) corresponding the rule given there.


==> counterex.tex <==
\emph{A Counterexample} \\
 Consider the following instance of Problem P1. We have equal prior on \(H\), that is \(P(H=0)=P(H=1)=1/2\). O1 has a time horizon of \(T^1=2\). Its observation space is \(\mathcal{Y}^1 = \{1,2,3\}\). The observations at time \(t=1\) follow the following conditional probabilities:
 \[ \begin{array}{lclr}
Observation & 1 & 2 & 3 \\
P(.|H=0)    & 0 & p & (1-p) \\
P(.|H=1)    & (1-p) & p & 0 
\end{array}\]
at time \(t=2\) follow the following conditional probabilities:
\[ \begin{array}{lclr}
Observation & 1 & 2 & 3 \\
P(.|H=0)    & 0 & q & (1-q) \\
P(.|H=1)    & (1-q) & q & 0 
\end{array}\]
Observe that O1's belief on \(H=0\)(\(\pi^1\)), only takes 3 possible values - \(0,1,1/2\).
O1 has to send a final message -\(0\) or \(1\)- to O2 by time \(t=2\). If O1 delays sending its final message to time \(t=2\), an additional cost \(c^1\) is incurred. After receiving a message from O1, observer 2 can either declare a decision on the hypothesis or take at most 1 more measurement of its own, that is, we have \(T^2 =1\). The measurements of O2 are assumed to be noiseless, so when O2 takes a measurement it knows exactly the value of \(H\). However, the measurement comes at a cost of \(c^2\). We will assume that \(J(U,H) =0\) if \(U=H\) and for the case of making a mistake \(U \neq H\), we assume that this cost is sufficiently high so that unless O2 is certain from O1's messages what the true hypothesis is, it will prefer taking a measurement at a cost \(c^2\) than making a guess. 
  At \(p=0.6\),\(c^2 > 6c^1\), it can be easily verified that the best threshold rule is described as follows:
  \begin{itemize}
  \item At \(t=1\), send \(0\) if \(\pi^1 = 1\), send \(1\) if \(\pi^1 =0\) and send \(b\) if \(\pi^1 = 1/2\).
  \item At \(t=2\), send \(0\) if \(\pi^1\) is either \(1\) or \(1/2\), send \(1\) otherwise.
  \end{itemize}
  If observer 2 receives \(0\) or \(1\) at time \(t=1\), it declares the received message as the final decision on the hypothesis. At \(t=2\), if O2 receives \(1\), it declares \(1\) as the final decision, otherwise it takes a measurement. Then the expected cost of this policy is given as: \( p(c^1 + c^2(1+q)/2)\) (since the system incurs a cost \(c^1\) with probability \(p\) and a cost \(c^2\) with probability \(p/2 + pq/2\)).
  \par
  Now consider the following non-threshold policy. 
  \begin{itemize}
  \item At \(t=1\), send \(0\) if \(\pi^1 = 1/2\), send \(b\) otherwise.
  \item At \(t=2\), send \(0\) if \(\pi^1\) is either \(1\) or \(1/2\), send \(1\) otherwise.
  \end{itemize}
  If observer 2 receives \(0\) at time \(t=1\), it takes a measurement and incurs a cost \(c^2\). If O2 receives a \(b\) at time \(t=1\), it waits for the final message at \(t=2\) and then declares the received message as its final decision on the hypothesis.  Then the expected cost of this policy is given as: \( pc^2 + (1-p)c^1\) (since the system incurs a cost \(c^2\) with probability \(p\) and a cost \(c^1\) with probability \(1-p\)). It is now easily seen that at \(p=0.6\) and \(c^2>6c^1\), if we choose \(q > 1-frac{2c^1}{3c^2}\), the non-threshold policy outperforms the best threshold policy.
  
 

==> hidden_slide.tex <==
\begin{frame}{Case B}
\begin{itemize}

\item<1-> The value function at \(T^2\) can be expressed as:
  \begin{equation}
  \tilde{V}_{T^2}(z^1_{1:T^1},\pi) := min\{ l^{0}(\pi), l^{1}(\pi)\}
  \end{equation}
  where \(l^{0}\) and \(l^{1}\) are affine functions of \(\pi\) that are independent of the choice of O1's policy \(\Gamma^1\).
  \item<2-> For a fixed policy \(\Gamma^1\) of O1, an optimal policy of O2 is of the form:
    \[ U^2_{T^2} = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^2_{T^2} \leq \alpha_{T^2}$} \\
               0 & \mbox{if $\pi^2_{T^2} > \alpha_{T^2}$ }
               \end{array}
               \right. \]
 \item<3-> Also, the value function at time \(k\) can be expressed as:
  \begin{equation}
  \tilde{V}_{k}(z^1_{1:k},\pi) := min\{ l^{0}(\pi), l^{1}(\pi), G_k(z^1_{1:k},\pi)\}
  \end{equation}
   where, for each realization \(z^1_{1:k}\) of messages from O1, \(G_k\) is a concave function of \(\pi\) that depends on the choice of O1's policy, \(\Gamma^1\).
   \item<4-> In this case, it can be 
\item<3-> Before receiving the final message, the optimal policy is characterized by a pair of time-varying thresholds.
\item<4-> After Sensor 2 receives the final message from Sensor 1, its problem is once again similar to the centralized Wald problem.
\end{itemize}
\end{frame}

==> mtns_detection.tex <==
\input preamble

\title
   {Decentralized Detection with Signaling}

\author
{Ashutosh Nayyar and Demosthenis Teneketzis\\
  Department of Electrical Engineering and Computer Science\\
  University of Michigan, Ann Arbor\\
  email: anayyar@umich.edu, teneket@eecs.umich.edu}

\begin{document}

\maketitle

%\begin{abstract}
 %We consider a sequential problem in decentralized detection. Two observers can make repeated noisy measurements
%of a binary hypothesis on the state of the environment. Initially, both the observers are operational, that is,  both observers continually take measurements of the state of the environment. Both the observers are faced with a stopping problem. At any time, any observer can decide to stop taking measurements and send a final message to the other observer or it may continue to take more measurements. Once an observer receives a message from the other observer, it is faced with a new stopping problem on whether to stop and declare a decision on the hypothesis or to continue taking measurements. The system incurs an accumulative operational cost that depends on the number of sensors that are taking measurements at a given time and a terminal cost that measures the accuracy of the final decision on the hypothesis. We compare this problem with the problem scenario where the observers only send their final messages to a fusion center that combines the two messages to produce a final decision (the decentralized Wald problem). We show that the presence of communication among the observers alters the nature of optimum stopping rules, that is, the optimal stopping rules are no longer characterized by two thresholds on the posterior belief on the hypothesis. We obtain new parametric characterization of optimal policies for the two observers.
%\end{abstract}

%\section{Introduction and Problem Formulation}
Decentralized detection problems are motivated by applications in decentralized systems such as sensor
networks and surveillance networks. In such networks, sensors receive different information about the environment
but share a common objective, for example to detect the presence of a target in a surveillance area. %Sensors may
%be allowed to communicate but they are constrained to exchange only a limited amount of information because of
%energy and other constraints.
 Inspired from the centralized sequential detection problem studied by Wald, a natural decentralized version of the sequential detection problem (called the decentralized Wald problem) involves two or more observers that sequentially make noisy measurements of the environment; the observers locally decide when to stop taking measurements and send a final binary message to a fusion center that combines these messages by a pre-specified rule (say, the majority rule). Thus, the decentralized Wald problem does not involve any communication among observers. A key result in this problem is that the optimal decision rules at different observers are characterized by two thresholds on the observer's posterior belief on the state of the environment. Even though these thresholds are coupled with each other (that is, the optimal choice of thresholds of one observer depends on the choice of thresholds at the other observers), the nature of the optimal decision rule is same as in the centralized one-observer problem.
\par
 We formulate a new version of a decentralized sequential detection problem where observers can communicate a final binary message to other observers. The presence of communication introduces signaling among the observers and alters the nature of optimal decision-rules. We consider a two hypothesis problem where the true hypothesis is modeled as a random variable $H$ taking values
$0$ or $1$ with known prior probabilities. We consider two observers: observer 1 (O1) and observer 2 (O2). We assume that each observer can make noisy
observations of the true hypothesis and that any two observations are conditionally independent given $H$.
\par
The $i^{th}$ observer observes the sequence $Y^i_t$, $t=1,2,\ldots$. At any time $t$, after having observed the sequence
of observations $Y^i_{1:t}$ (that is, $Y^i_1,Y^i_2,\ldots,Y^i_t$), observer $i$ can decide either to stop and send a binary message 0 or 1 to the other observer or to
postpone its decision and get another measurement. After one of the observers has sent its final message, it stops operating. The other observer is then faced with a new stopping problem. At each time instant, it can decide either to stop and declare a final decision on the hypothesis or take another measurement. We denote by $U^i_t$ the decision of the $i^{th}$ observer at time $t$. $U^i_t$ belongs to the set $\{0,1,b\}$, where $b$ denotes a blank, that is, no message. We have,
 \begin{equation}
 U^i_t = \gamma^i_t(Y^i_{1:t},U^1_{1:t-1},U^2_{1:t-1})
 \end{equation}
 where the collection of functions $\Gamma^i:=(\gamma^i_t$, $t=1,2,\ldots)$ constitute the policy of the $i^{th}$ observer. We define the following stopping times:
\[\tau^1 := min\{t:U^1_t \neq b\}\]
\[\tau^2 := min\{t:U^2_t \neq b\}\]
We further define, $ ~~\tau^{min} := min\{\tau^1,\tau^2\}$, $\tau^{max} := max\{\tau^1,\tau^2\} $ and
\[L:= \left\{ \begin{array}{l} 1 \mbox{~~~if~~~} \tau^2 < \tau^1 \\
                               2 \mbox{~~~if~~~} \tau^2 \geq \tau^1 \end{array} \]
The system incurs a total cost given by:
 \begin{equation}
  J(\Gamma^1, \Gamma^2):= \mathds{E}^{\Gamma^1,\Gamma^2}\{K\tau^{min} + k(\tau^{max}-\tau^{min}) + J(U^{L}_{\tau^{max}},H)\}
 \end{equation}    
 where $K>k>0$ are constants and $J(\cdot,\cdot)$ is a distortion function. The first term in the cost represents the operating costs when both observers are active, the second term represents the operating cost of only one observer and the last term represents the accuracy of the final decision. The objective is to select policies $\Gamma^1,\Gamma^2$ that minimize the total expected cost. 
 \par
 We identify information states for the two observers and provide a parametric characterization of optimal policies. We show that a two-threshold rule on the posterior belief is no longer optimal. Instead the optimal rules are characterized by four thesholds until one of the observers sends its final message. After one observer has sent its final message, the other observer employs a two threshold rule to make its decision.
 %\section{Results}




%\bibliographystyle{IEEEtran}
%\bibliography{IEEEabrv,collection}

\end{document} 

==> multi-sensor.tex <==
\section{Extension to Multiple Sensors} \label{sec:MS}
      In this section, we extend our  results to the case when several peripheral sensors similar to observer 1 in  Problems P1 and P2 are required to send a single final message to a coordinating sensor (similar to O2) which may be taking its own measurements. We show that the peripheral sensors have similar parametric characterizations of their optimal policies as O1 in Problems P1 and P2. We obtain a characterization of coordinator's strategy that is similar to that of O2.
      \par  
     Consider a group of N peripheral sensors: S1,S2,...,SN and a coordinating sensor S0. Each sensor can make repeated observations on the random variable \(H\). As before, we will assume that conditioned on \(H\), the observations at  different sensors are independent and the observations made at different time instants  at any sensor are also independent conditioned on \(H\). 
     \begin{figure}[ht]
\begin{center}

\includegraphics[height=5cm,width=7cm]{dd_new_v2.pdf}
\caption{Decentralized Detection with N Peripheral Sensors and 1 Coordinating Sensor}
%\end{center}

\end{center} 
\end{figure}
     \par
      Each of the peripheral sensors observes its own measurement process \(Y^i_t,i=1,2...,N\) and \(t=1,2,...\). At any time \(t\), the \(i^{th}\) peripheral sensor can decide either to stop and send a binary message \(0\) or \(1\) to the coordinating sensor or to continue taking measurements. Each time the \(i^{th}\) sensor decides to continue taking measurements, a cost \(c^i\) is incurred. Each peripheral sensor sends only a single final message to the coordinator. The policy of \(i^{th}\) sensor is of the form:
      \begin{equation}\label{eq:MS1}
      Z^i_t = \gamma^i_t(Y^i_{1:t})
      \end{equation}
      where \(Z^i_t\) is \(i^{th}\) sensor's  message at time \(t\) to the coordinating sensor. \(Z^1_t\) belongs to the set \(\{0,1,b\}\), where we use \(b\) for blank message, that is, no transmission. The sequence of functions \(\Gamma^i =(\gamma^i_1,\gamma^i_2,...)\) is the policy of the \(i^{th}\) sensor. \(\tau^i\) is the stopping time when \(i^{th}\) sensor sends a final message to the coordinating sensor, that is,
\begin{equation} \label{eq:MS1.2}
 \tau^i=min\{t: Z^i_t \in \{0,1\}\}
\end{equation}
The coordinating sensor observes its own measurement process, \(Y^0_t,t=1,2,...\). In addition, it receives messages from all the peripheral sensors (we assume that when the coordinating sensor receives a message it knows which peripheral sensor sent that message). At any time \(t\), S0 can decide to stop and declare a final decision on the hypothesis or take a new measurement and wait for more messages from the peripheral sensors. Each time S0 postpones its decision on the hypothesis, it incurs a cost \(c^0\). When S0 announces a final decision \(U\) on the hypothesis, it incurs a cost given as \(J(U,H)\). Thus, the coordinator's decision at time \(t\) is given as:
\begin{equation}
 U_t = \gamma^0_t(Y^0_{1:t}, Z^1_{1:t},Z^2_{1:t},...,Z^N_{1:t})
\end{equation}
\(U_t\) belongs to the set \(\{0,1,N\}\), where we use \(N\) for a null decision, that is, a decision to continue waiting for more messages and taking more measurements. The sequence of functions \(\Gamma^0 =(\gamma^0_1,\gamma^0_2,...)\) is the policy of the coordinating sensor.  \(\tau^0\) is the stopping time when S0 announces its final decision on the hypothesis, that is,
\begin{equation} \label{eq:MS5.1}
 \tau^0=min\{t: U_t \in \{0,1\}\}
\end{equation}
\emph{Problem P3:} Consider a finite horizon \(T^i\) for the peripheral sensors (that is, we require that \(\tau^i \leq T^i\)) and a finite horizon \(T^0\) for the coordinating sensor, that is, \(\tau^0 \leq T^0\). The optimization problem is to select polices \(\Gamma^0, \Gamma^1,..,.\Gamma^N\) of all the sensors to minimize
\begin{equation}\label{eq:MSobj}
\mathds{E}\{\sum_{i=0}^{N}c^i.\tau^i + J(U_{\tau^0},H)\}
\end{equation}
\par
    We now obtain a characterization of the peripheral sensor's optimal policies. For the \(i^{th}\) peripheral sensor, we define
    \begin{equation}
      \pi^i_t(Y^i_{1:t}) := P(H=0|Y^i_{1:t})
     \end{equation}
\begin{theorem}
      For any peripheral sensor \(i\) and any fixed choice of strategies \(\Gamma^j,\) for \(j=0,1,...,N,j \neq i\), there is an optimal policy of the peripheral sensor \(i\) of the form:
      \[ Z^i_{T^i} = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^i_{T^i} \leq \alpha^i_{T^i}$} \\
               0 & \mbox{if $\pi^i_{T^i} > \alpha^i_{T^i}$ }
               \end{array}
               \right. \]
               where \(0 \leq \alpha^i_{T^i} \leq 1\)  and for \(k=1,2,..,T^i-1\),
         \[ Z^i_k = \left \{ \begin{array}{ll}
               b & \mbox{if $\pi^i_k < \alpha^i_k$}  \\
               1 & \mbox{if $\alpha^i_k \leq \pi^i_k \leq \beta^i_k$} \\
               b & \mbox{if $\beta^i_k<\pi^i_k< \delta^i_k$} \\
               0 & \mbox{if $\delta^i_k \leq \pi^i_k \leq \theta^i_k$} \\
               b & \mbox{if $\pi^i_k > \theta^i_k$}
               \end{array}
               \right. \]  
               where \(0 \leq \alpha^i_k \leq \beta^i_k \leq \delta^i_k \leq \theta^i_k \leq 1\). 
\end{theorem}
\begin{IEEEproof}
             The main idea of the proof is that once the policies of all sensors except \(i\) are fixed, the optimization problem for the \(i^{th}\) sensor is similar to the problem for O1 in Problem P2. The \(i^{th}\) sensor plays the role of O1 in Problem P2 and the coordinating sensor plays the role of O2. The observations of the coordinating sensor at time \(t\) can be defined as:
             \[ \tilde{Y}^0_t := (Y^0_t,Z^j_t,j=1,2,...,N,j \neq i)\]
             Note that conditioned on \(H\), the observations \(\tilde{Y}^0_t\) are independent of the \(i^{th}\) sensor's observations. We can now follow the arguments of Theorem 1 and 2 to conclude the result for the \(i^{th}\) peripheral sensor. We refer the reader to [8] for a detailed proof. 
\end{IEEEproof}
\par
        To find a characterization of the coordinating sensor's policy, we fix the policies of all peripheral sensors and define
        \begin{align} &\pi^0_t(Y^0_{1:t},Z^1_{1:t},Z^2_{1:t},...,Z^N_{1:t}) \nonumber \\ &:= P(H=0|Y^0_{1:t},Z^1_{1:t},Z^2_{1:t},...,Z^N_{1:t}) \end{align}
\begin{theorem}
     For any fixed choice of policies of the peripheral sensors, the policy of the coordinating sensor is given as 
     \[ U_{T^0} = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^0_{T^0} \leq \alpha_{T^0}$} \\
               0 & \mbox{if $\pi^0_{T^0} > \alpha_{T^0}$ }
               \end{array}
               \right. \]
   \[ U_k = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^0_k \leq \alpha_k(Z^1_{1:k},Z^2_{1:k},...,Z^N_{1:k})$}  \\
               N & \mbox{if $\alpha_k(Z^1_{1:k},Z^2_{1:k},...,Z^N_{1:k}) < \pi^0_k <$} \\ & \mbox{$\beta_k(Z^1_{1:k},Z^2_{1:k},...,Z^N_{1:k})$} \\
               0 & \mbox{if $\pi^0_k \geq \beta_k(Z^1_{1:k},Z^2_{1:k},...,Z^N_{1:k})$}
               \end{array}
               \right. \] 
               where \(0\leq\alpha_k(Z^1_{1:k},Z^2_{1:k},...,Z^N_{1:k})\)\(\leq \beta_k(Z^1_{1:k},Z^2_{1:k},...,Z^N_{1:k})\leq 1\) are thresholds that depend on sequence of messages received from the peripheral sensors.
\end{theorem}
\begin{IEEEproof}
  The proof follows the arguments of Theorem 3 and Theorem 4. See [8].
\end{IEEEproof}


==> qualitative_properties_2.tex <==
\section{Qualitative Properties for O2} \label{sec:QP2}

\subsection{Problem P1}
Consider a fixed policy \(\Gamma^1 = (\gamma^1_1,\gamma^1_2,...,\gamma^1_{T^1})\) for O1. Then, after O1 sends its final message, we can define the following probability for O2:
\[\pi^2_0 := P^{\Gamma^1}(H=0|Z^1_{1:\tau^1}) \]
This is O2's belief on the true hypothesis after having observed the messages from O1 (that is a sequence of \(\tau^1-1\) blanks and a final \(Z^1_{\tau^1} \in \{0,1\}\)). Now, the optimization problem for O2 is the classical centralized Wald problem with the prior probability given by \(\pi^2_0\). It is well-known that the optimal policy for Wald problem is a rule of the form:
%\[ U^2_{T^2} = \left \{ \begin{array}{ll}
 %              0 & \mbox{if $\pi^2_{T^2} \leq  w_{T^2}$} \\
  %             1 & \mbox{if $\pi^2_{T^2} >  w_{T^2} $}
   %            \end{array}
    %           \right. \]  
%and   
\[\hspace{20pt} U^2_k = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^2_k \leq w^1_k$} \\
               N & \mbox{if $w^1_k<\pi^2_k<w^2_k$} \\
               0 & \mbox{if $\pi^2_k \geq w^2_k$}
               \end{array}
               \right. \]               
   where \(\pi^2_k\) is the belief on hypothesis after \(k\) observations, 
   \[ \pi^2_k(Y^2_{1:k}) := P^{\Gamma^1}(H=0|Z^1_{1:\tau^1},Y^2_{1:k})\] 
   \[ = \frac{P(Y^2_{1:k}|H=0).\pi^2_0}{P(Y^2_{1:k}|H=0).\pi^2_0+P(Y^2_{1:k}|H=1).(1-\pi^2_0)} \]
and \(w^1_k \leq w^2_k\), for \(k=1,2,..,T^2-1\) and \(w^1_{T^2} = w^2_{T^2}\).   
 %  Note that in the Wald problem, the thresholds \(w^1_k,w^2_k\) depend only on the cost parameters \(c^2\) and \(J(U^2,H)\) and not on the prior %probabilities [\textbf{Thresholds on likelihood ratio, as described in Wald's book depend on prior...but the thresholds on pi do not}]. 
              


\subsection{Information State in Problem P2}
  Consider a fixed policy \(\Gamma^1 = (\gamma^1_1,\gamma^1_2,...,\gamma^1_{T^1})\) for O1. Define the following probability for O2:
  \[ \pi^2_t(Y^2_{1:t},Z^1_{1:t}) := P^{\Gamma^1}(H=0|Y^2_{1:t},Z^1_{1:t}) \]
   \(\pi^2_t\) is the observer 2's belief on the hypothesis based on its observations till time \(t\) and the messages received from O1 till time \(t\) (where the messages from O1 could be all blanks or some blanks terminated by a \(0\) or \(1\)). For \(t=0\), we have \(\pi^2_0 = p_0\).\\ 
The following theorem shows that \(\pi^2_t\) and \(Z^1_{1:t}\) together form an information state for O2.
 \begin{theorem}
  In Problem P2, with a fixed policy \(\Gamma^1\) of O1, there is an optimal policy for O2 of the form:
  \begin{equation} \label{eq:Qp21}
  U^2_t = \gamma^2_t(Z^1_{1:t},\pi^2_t)
  \end{equation}
  for \(t=1,2,...,T^2\). Moreover, this optimal policy can be determined by the following dynamic program:
  \begin{align}
  	\tilde{V}_{T^2}(Z^1_{1:T^1},\pi) := min \{ &E^{\Gamma^1} [J(0,H)|\pi^2_{T^2}=\pi], \nonumber \\
  	                                  &E^{\Gamma^1} [J(1,H)|\pi^2_{T^2}=\pi]  \} \label{eq:Qp22.1}
  \end{align}
  and for \(k=(T^1-1),...,1\),
  \begin{align}
   &\tilde{V}_k(Z^1_{1:k},\pi) := min \{ \nonumber \\
   &E^{\Gamma^1} [J(0,H)|\pi^2_{k}=\pi], \nonumber \\
  	                                  &E^{\Gamma^1} [J(1,H)|\pi^2_{k}=\pi], \nonumber \\
  	                                  & c^2 + E^{\Gamma^1} [\tilde{V}_{k+1}(Z^1_{1:k+1},\pi^2_{k+1})|\pi^2_{k}=\pi,Z^1_{1:k}]\} \label{eq:Qp22.2}
  \end{align}
 \end{theorem}    
\begin{IEEEproof}
  See Appendix B.
\end{IEEEproof}
\par
 Observe that in the last term of (\ref{eq:Qp22.2}), which corresponds to the cost of postponing the final decision at time \(k\), we have \(\pi^2_k\) as well as all messages from O1 in the conditioning variables. It is because of this term  that we need the entire sequence of messages as a part of the information state. To intuitively see why these messages are needed in the conditioning, note that the cost of continuing depends on future messages from O1. In order to form a belief on future messages, O2 needs a belief on the hypothesis and (since  O1 has perfect recall) a belief on all observations of O1 so far.  Clearly, the messages received till time \(k\) provide information about the observations of O1 till time \(k\) and are therefore included in the information state.
 \par
 We can now prove the following lemma about the value functions \(\tilde{V}_k\).
 \begin{lemma}
 The value function at \(T^2\) can be expressed as:
  \begin{equation}
  \tilde{V}_{T^2}(z^1_{1:T^1},\pi) := min\{ l^{0}(\pi), l^{1}(\pi)\}
  \end{equation}
  where \(l^{0}\) and \(l^{1}\) are affine functions of \(\pi\) that are independent of the choice of O1's policy \(\Gamma^1\).
  Also, the value function at time \(k\) can be expressed as:
  \begin{equation}
  \tilde{V}_{k}(z^1_{1:k},\pi) := min\{ l^{0}(\pi), l^{1}(\pi), G_k(z^1_{1:k},\pi)\}
  \end{equation}
   where, for each realization \(z^1_{1:k}\) of messages from O1, \(G_k\) is a concave function of \(\pi\) that depends on the choice of O1's policy, \(\Gamma^1\).
 \end{lemma}
 \begin{IEEEproof}
 See Appendix C.
 \end{IEEEproof}
 \begin{theorem}
   For a fixed policy \(\Gamma^1\) of O1, an optimal policy of O2 is of the form:
    \[ U^2_{T^2} = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^2_{T^2} \leq \alpha_{T^2}$} \\
               0 & \mbox{if $\pi^2_{T^2} > \alpha_{T^2}$ }
               \end{array}
               \right. \]
   \[ U^2_k = \left \{ \begin{array}{ll}
               1 & \mbox{if $\pi^2_k \leq \alpha_k(Z^1_{1:k})$}  \\
               N & \mbox{if $\alpha_k(Z^1_{1:k}) < \pi^1_k < \beta_k(Z^1_{1:k})$} \\
               0 & \mbox{if $\pi^1_k \geq \beta_k(Z^1_{1:k})$}
               \end{array}
               \right. \] 
               where \(0 \leq \alpha_k(Z^1_{1:k}) \leq \beta_k(Z^1_{1:k}) \leq 1\) are thresholds that depend on sequence of messages received from O1 (\(Z^1_{1:k}\)).
 \end{theorem}
 \begin{IEEEproof}
     At any time \(k\), if \(\pi^2_k = 0\), then it is optimal to stop and declare the hypothesis to be \(1\) since cost of continuing will be at least \(c^2+J(1,1)\) which is more than \(J(1,1)\) -the cost of immediately stopping and declaring \(U^2_k =1\). Similarly, at \(\pi^2_k = 1\), it is optimal to stop and declare \(U^2_k=0\). These observations along with Lemma 2 imply the result of the theorem. 
 \end{IEEEproof}
          
          		Thus, according to Theorem 4, the thresholds to be used at time \(k\) by O2 depend on the sequence of messages received from O1 time \(k\). This kind of parametric characterization may not appear very appealing since for each time \(k\) one may have to know a number of possible thresholds - one for each possible realization of messages \(z^1_{1:k}\). We will now argue that there is in fact a simple representation of the thresholds. Note that after time \(\tau^1\), when O1 sends a final message, O2 is faced with a classical Wald problem with an available time-horizon of \(T^2-\tau^1\). Now suppose that the classical Wald thresholds are available for a time horizon of length \(T^2\) -lets call these \((w^1_1,w^2_1),(w^1_2,w^2_2),...,w_{T^2}\). Then the Wald thresholds for a problem with time horizon \(T^2-\tau^1\) are simply \((w^1_{\tau^1+1},w^2_{\tau^1+1}),(w^1_{\tau^1+2},w^2_{\tau^1+2}),...,w_{T^2}\). Thus, once  O2 hears a final message from O1, it starts using the classical Wald thresholds from that time onwards. In other words, O2 operation is described by the following simple algorithm: 
   \begin{itemize}
   \item From time \(k=1\) onwards, the optimal policy is to use a threshold rule given by 2 numbers \(\alpha_k(b_{1:k})\) and \(\beta_k(b_{1:k})\), \emph{until O1 sends its final message \(Z^1_k \in \{0,1\}\).} (As before, \(b_{1:k}\) stands for sequence of \(k\) blank messages.)
   \item From the time O1 sends a final message, start using Wald thresholds \((w^1_k,w^2_k),...,w_{T^2}\).
   \end{itemize}
          		   Thus O2's optimal policy is completely characterized by just two tables of thresholds: \([(\alpha_1(b_{1:1}),\beta_1(b_{1:1}))\), \((\alpha_2(b_{1:2}),\beta_2(b_{1:2})),...,(\alpha_{T^1}(b_{1:T^1}),\beta_{T^1}(b_{1:T^1}))]\) and the Wald thresholds \([(w^1_1,w^2_1),(w^1_2,w^2_2),...,w_{T^2}]\) . 
     
 
 
 
 

==> references.tex <==
\begin{thebibliography}{20}
\bibitem{Sandell} Tenney, R. R., and Sandell, N. R. Jr., ``Detection with distributed sensors'', \textit{IEEE Trans. Aerospace Electron. Systems} \textbf{AES-17}(4), 1981, pp.501-510.
\bibitem{Teneket} Teneketzis D., and Ho Y.C., ``The Decentralized Wald Problem'', \textit{Information and Computation},\textbf{73}, 1987, pp. 23-44.

\bibitem{Tsitsiklis} Tsitsiklis J. N., ``Decentralized detection,'' \textit{Adv. Statist. Signal Processing},
vol. 2, pp. 297–344, 1993. 
\bibitem{Tsitsiklis2} Tsitsiklis J. N., ``On Threshold Rules in Decentralized detection,'' in \textit{Proc. 25th IEEE Conf. Decision and Control}, Athens, Greece, 1986, pp. 232-236.
vol. 2, pp. 297–344, 1993. 
\bibitem{Veeravalli} Veeravalli V. V., Basar T., and Poor H.V., ``Decentralized sequential detection
with a fusion center performing the sequential test,'' \textit{IEEE Trans.
Inform. Theory}, vol. 39, pp. 433–442, Mar. 1993.
\bibitem{Veeravalli2} Chamberland J.F., and Veeravalli V. V., `` Asymptotic results for decentralized detection in power-constrained wireless
sensor networks,'' \textit{IEEE Trans. Signal Processing}, vol. 51, no. 2, pp. 407–416, February 2003.
\bibitem{Wald} Wald, A., `` \textit{Sequential Analysis}'', Wiley, New York, 1947.
\bibitem{Ashutosh} Nayyar A., and Teneketzis D., ``A sequential Problem in Decentralized Detection '', Control Group Report CGR-09-03, Department of EECS, University of Michigan, Ann Arbor, MI 48109.
\end{thebibliography}


==> temp.tex <==

\begin{frame}{A non-threshold rule}
 \begin{itemize}
    \item<1-> Consider the following non-threshold rule:
\begin{columns}[t]
 \begin{column}{5cm}
 At \(t=1\), 
 \[ Z^1_1 = \left \{ \begin{array}{ll}
               0 & \mbox{if $\pi^1_1 = 0 $} \\
               & \mbox{} \\
               1 & \mbox{if $\pi^1_1 = 1/2 $} \\
               & \mbox{} \\
               b & \mbox{if $\pi^1_1 = 1$}
               \end{array}
               \right. \]
 
 \end{column}
 \begin{column}{5cm}
  At \(t=2\),
 \[ Z^1_2 = \left \{ \begin{array}{ll}
               0 & \mbox{if $\pi^1_2 < 1 $} \\
               & \mbox{}\\
               1 & \mbox{if $\pi^1_2 = 1$}
               \end{array}
               \right. \] 
 \end{column}
 \end{columns}
 \item<2-> Sensor 2's rule is: 
 \begin{itemize} 
  \item<2->At \(t=1\), if the received message is \(0\), declare \(U^2 =0\).
  \item<2-> At \(t=1\), if the received message is \(1\), take a measurement.
  \item<2-> Else wait to hear the message at \(t=2\), declare the received messages as the final decision \(U^2 = Z^1_2\).
 \end{itemize}
 \item<3-> Expected cost of this policy: \(pc^2 + (1-p)c^1/2\)
 \item<4-> Cost of non-threshold rule < Cost of Best threshold rule for \(q\) large enough.
\end{itemize} 
\end{frame}
\begin{frame}
\begin{itemize}
\item<1-> A final message from Sensor 1 need not be its final decision on \(H\)
\item<2-> At certain times, a blank message may be used to convey certainty about \(H\).
\item<3-> In the decentralized Wald problem, it was optimal for each sensor to covey its final decision to the fusion center.
\item<4-> In Problems P1 and P2, Sensor 1 may try to convey information about its belief.
\item<5-> For example, if at time \(t\), S1 is very certain about \(H\), and it is able to convey that it is certain, then it can prevent S2 from taking many more measurements.
\item<6-> On the other hand, if S1 is very doubtful, a terminal message may prompt S2 to make its own measurement instead of waiting for S1's message.
\end{itemize}
\end{frame}
\begin{frame}{Parametric Characterization}
\begin{itemize}
\item<1-> With a fixed (but arbitrary) choice of \(\Gamma^2\), the value function at \(T^1\) can be expressed as:
  \begin{equation}
  V_{T^1}(\pi) := min\{ L^{0}_{T^1}(\pi), L^{1}_{T^1}(\pi)\}
  \end{equation}
  where \(L^{0}_{T^1}\) and \(L^{1}_{T^1}\) are affine functions of \(\pi\) that depend on the choice of O2's policy \(\Gamma^2\).
\item<2-> Consequently, an optimal policy at time \(T^1\) is of the form:
       \[ Z^1_{T^1} = \left \{ \begin{array}{ll}
               0 & \mbox{if $\pi^1_{T^1} \leq \alpha_{T^1}$} \\
               1 & \mbox{if $\pi^1_{T^1} > \alpha_{T^1}$ }
               \end{array}
               \right. \]  
\item<3-> Also, the value function at time \(k\) can be expressed as:
  \begin{equation}\label{eq:PFlemma1}
  V_{k}(\pi) := min\{ L^{0}_k(\pi), L^{1}_k(\pi), G_k(\pi)\}
  \end{equation}
  where \(L^{0}_{k}\) and \(L^{1}_{k}\) are affine functions of \(\pi\) and \(G_k\) is a concave function of \(\pi\) that depend on the choice of \(\Gamma^2\).
\item<4->  Consequently, an optimal policy for \(t < T^1\) is described by at most 4 thresholds:
    \[ Z^1_k = \left \{ \begin{array}{ll}
               b & \mbox{if $\pi^1_k < \alpha_k$}  \\
               0 & \mbox{if $\alpha_k \leq \pi^1_k \leq \beta_k$} \\
               b & \mbox{if $\beta_k<\pi^1_k < \delta_k$} \\
               1 & \mbox{if $\delta_k \leq \pi^1_k \leq \theta_k$} \\
               b & \mbox{if $\pi^1_k > \theta_k$}
               \end{array}
               \right. \]    
\end{itemize}
\end{frame}


\begin{frame}{Structural Results for Sensor 2}
\uncover<1->{ \structure{\textcolor{darkblue}{Case A:}}}
\begin{itemize}
\item<1-> Sensor 2 waits for S1's final message before starting its own measurements.
\item<2-> Consider a fixed policy \(\Gamma^1\) of sensor 1.
\item<3-> After Sensor 2 receives the final message from Sensor 1, its belief is:
\[ \pi^2_0 := P^{\Gamma^1}(H=1|Z^1_{1:\tau^1}) \]
\item<4-> Sensor 2 problem is now a centralized Wald problem with \(\pi^2_0\) as the starting belief for which optimal policy is a classical 2-threshold rule.
\end{itemize}
\end{frame}
\begin{frame}{Structural Results for Sensor 2 Contd.}
\uncover<1->{ \structure{\textcolor{darkblue}{Case B:}}}
\begin{itemize}
\item<1-> Sensor 2 is taking measurements from \(t=1\).
\item<2-> Consider a fixed policy \(\Gamma^1\) of sensor 1.
\item<3-> Information state for sensor 2 : \((Z^1_{1:t},\pi^2_t)\), where
\[ \pi^2_t := P^{\Gamma^1}(H=0|Y^2_{1:t},Z^1_{1:t}) \]
\item<4->Dynamic program:
  \begin{align}
  	\tilde{V}_{T^2}(Z^1_{1:T^1},\pi) := min \{ &E^{\Gamma^1} [J(0,H)|\pi^2_{T^2}=\pi], \nonumber \\
  	                                  &E^{\Gamma^1} [J(1,H)|\pi^2_{T^2}=\pi]  \} \label{eq:Qp22.1}
  \end{align}
  and for \(k=(T^1-1),...,1\),
  \begin{align}
   \tilde{V}_k(Z^1_{1:k},\pi) := min \{ &E^{\Gamma^1} [J(0,H)|\pi^2_{k}=\pi], \nonumber \\
  	                                  &E^{\Gamma^1} [J(1,H)|\pi^2_{k}=\pi], \nonumber \\
  	                                  & c^2 + E^{\Gamma^1} [\tilde{V}_{k+1}(Z^1_{1:k+1},\pi^2_{k+1})|\pi^2_{k}=\pi,Z^1_{1:k}]\} \label{eq:Qp22.2}
  \end{align}
\end{itemize}
\end{frame}\begin{frame}
\begin{itemize}
\item<1-> After Sensor 2 receives the final message from Sensor 1, its problem is once again similar to the centralized Wald problem.
\item<2-> The value function at \(T^2\) can be expressed as:
  \begin{equation}
  \tilde{V}_{T^2}(z^1_{1:T^1},\pi) := min\{ l^{0}(\pi), l^{1}(\pi)\}
  \end{equation}
  where \(l^{0}\) and \(l^{1}\) are affine functions of \(\pi\) that are independent of the choice of O1's policy \(\Gamma^1\).
 \item<3-> Also, the value function at time \(k\) can be expressed as:
  \begin{equation}
  \tilde{V}_{k}(z^1_{1:k},\pi) := min\{ l^{0}(\pi), l^{1}(\pi), G_k(z^1_{1:k},\pi)\}
  \end{equation}
   where, for each realization \(z^1_{1:k}\) of messages from O1, \(G_k\) is a concave function of \(\pi\) that depends on the choice of O1's policy, \(\Gamma^1\).
\item<3-> Before receiving the final message, the optimal policy is characterized by a pair of time-varying thresholds.
\end{itemize}
\end{frame}
\section{Extensions}
\begin{frame}{Extensions}
\begin{figure}
  \includegraphics[height=1.7cm,width=4.5cm]{dd_new_v2.pdf} 
   \end{figure}
   \begin{itemize}
   \item<1-> Multiple peripheral sensors \(P_1,,...,P_N\) and a coordinating sensor \(C_0\).
   \item<2-> All sensors make conditionally independent observations.
   \item<3-> Peripheral Sensors can choose to stop and send a final message to the coordinating sensor.
   \item<4-> Coordinating sensor has a stopping problem: it can choose to stop and declare a decision\\
   or continue to make more measurements and receive more messages.
   \item<5-> Finite horizon for all sensors.
   \end{itemize}
\end{frame}
\begin{frame}{Optimization Problem}
\begin{itemize}
 \item<1-> Optimization problem is to select polices \(\Gamma^0, \Gamma^1,..,.\Gamma^N\) of all the sensors to minimize
\begin{equation}\label{eq:MSobj}
\mathds{E}\{\sum_{i=0}^{N}c^i.\tau^i + J(U_{\tau^0},H)\}
\end{equation}
where \(\tau^i\)s are stopping times of the sensors.
\item<2-> For fixed policies of all but one peripheral sensors, the problem reduces to Sensor 1's problem in P2.
\item<3-> Optimal rules characterized by 4 thresholds for the peripheral sensors.
\item<4-> Optimal rules of coordinating sensor characterized by 2 thresholds that depend on the messages received.
\end{itemize}
\end{frame}
\section{Conclusions}
\begin{frame}{Conclusions}
\begin{itemize}

\item<1->  We considered a new sequential problem in decentralized detection.
\item<2-> Communication among sensors implied a dynamic team problem.
\item<3-> Classical Wald-like thresholds are no longer optimal.
\item<4-> However, there is a parametric characterization available.

\end{itemize}
\end{frame}

==> temp_counter.tex <==
We will show by means of a counterexample that such a structure is not necessarily optimal for observer 1. 
 Consider the following instance of problem P1. Observer 1 has a time horizon of \(T^1=2\). Its observations at \(t=1\) are given by the following conditional probabilities.  
\[ \begin{array}{lclcr}
Observation & 1 & 2 & 3 & 4 \\
P(.|H=0)    & 0 & p/3 & 2p/3 & (1-p) \\
P(.|H=1)    & (1-p) & 2p/3 & p/3 & 0 
\end{array}\]
O1's observations at time \(t=2\) are just noise and give no new information. Note that the observations are indexed in order of the posterior belief \(\pi^1\) they generate, that is, \(P(H=0|Observation 1) < P(H=0|Observation 2)\) and so on. If O1 delays sending its final message to time \(t=2\), it has to pay a cost of \(c^1\). Observer 2 can make a noiseless measurement at a cost of \(c^2\). Observer 2's cost of making a wrong decision is chosen sufficiently high so that unless it is certain from O1's message what the true hypothesis is, O2 will prefer taking a measurement at a cost \(c^2\) than making a guess.
It can be shown that for equal prior (\( p_0 =1/2\)), \(c^2>2c^1\) and \(1/2<p<1\), a non-threshold rule for O1 (given below) performs better than any threshold policy. 
\begin{itemize}
\item At \(t=1\), send \(0\) if observation 2 occurs and \(1\) if observation 3 occurs. Send a blank otherwise otherwise.
\item At \(t=2\), send \(1\) if the posterior belief on \((H=0)\) is less than \(1/2\) and \(0\) otherwise.
\end{itemize}

==> temp_information_states.tex <==
For $t=T-1,T-2,\ldots,1$,
%\begin{align}
%V_t(\pi,1) = \left \{ \begin{array}{ll}
%               &E[J(0,H)|\Pi^2_{t}=\pi], \nonumber \\
%  	                                  &E[J(1,H)|\Pi^2_{t}=\pi], \nonumber \\
% 	                                  &k+ E[V{t+1}(\Pi_{t+1},1)|\Pi^2_{t}=\pi,\ind_{\{\tau^1<t\}=1}]\}
%               \end{array}
%               \right.
%\end{align}               
\begin{align}
V_t(\pi,0) = \left \{ \begin{array}{ll}
               %&E[\ind_{\{\tau^1=t\}}J(0,H) + \ind_{\{\tau^1>t\}}(k(\tau^1-t)+ J(U^1_{\tau^1},H))|\Pi^2_{t}=\pi,U^2_t=0], \nonumber \\
  	                                  %&E[\ind_{\{\tau^1=t\}}J(1,H) + \ind_{\{\tau^1>t\}}(k(\tau^1-t)+ J(U^1_{\tau^1},H))|\Pi^2_{t}=\pi,U^2_t=1], \nonumber \\
  	                                 % &\ind_{\{\tau^1=t\}}(k+E[V{t+1}(\Pi_{t+1},1)|\Pi^2_{t}=\pi,\ind_{\{\tau^1<t\}=0}]) \nonumber \\
  	                                 % &+\ind_{\{\tau^1>t\}}(K+E[V{t+1}(\Pi_{t+1},0)|\Pi^2_{t}=\pi,\ind_{\{\tau^1<t\}=0}]) 
  	                               
               \end{array}
               \right.
\end{align}               
%\end{definition}

 \begin{theorem}
  In Problem P2, with a fixed policy \(\Gamma^1\) of O1, there is an optimal policy for O2 of the form:
  \begin{equation} \label{eq:Qp21}
  U^2_t = \gamma^2_t(\Theta_t) = \gamma^2_t(\Pi^2_t,\ind_{\{\tau^1<t\}}) 
  \end{equation}
  for \(t=1,2,...,T\). Moreover, this optimal policy can be determined by the following dynamic program:\\
  
 
\begin{align}
   &V_T(\pi,a) := min \{ \nonumber \\
   &E[J(0,H)|\Pi^2_{T}=\pi], \nonumber \\
  	                                  &E[J(1,H)|\Pi^2_{T}=\pi]
\end{align}
where $\pi \in [0,1]$, $a \in \{0,1\}$. The optimal policy at time $T$ for observer 2 is given by selecting the minimizing term for each realizations of $\pi$ and $a$, where selecting the first term corresponds to $U^2_T =0$ and selecting the second corresponds to $U^2_T =1$. 

For $t=T-1,T-2,\ldots,1$  	                                  

\begin{align}
   &V_t(\pi,a) := min \{ \nonumber \\
   &E[J(0,H)|\Pi^2_{t}=\pi], \nonumber \\
  	                                  &E[J(1,H)|\Pi^2_{t}=\pi], \nonumber \\
  	                                  & E[K + (k-K)\ind_{\{\tau^1<t\}} + V{t+1}(\Theta_{t+1})|\Pi^2_{t}=\pi,\ind_{\{\tau^1<t\}=a}]\} \label{eq:dp1.1}
  \end{align}
The optimal policy at time $t$ for observer 2 is given by selecting the minimizing term for each realizations of $\pi$ and $a$, where selecting the first term corresponds to $U^2_t =0$, the second corresponds to $U^2_t =1$ and the last term corresponds to $U^2_t =b$.
 \end{theorem}    
\begin{IEEEproof}
  See Appendix B.
\end{IEEEproof}
\par
 Observe that in the last term of (\ref{eq:Qp22.2}), which corresponds to the cost of postponing the final decision at time \(k\), we have \(\pi^2_k\) as well as all messages from O1 in the conditioning variables. It is because of this term  that we need the entire sequence of messages as a part of the information state. To intuitively see why these messages are needed in the conditioning, note that the cost of continuing depends on future messages from O1. In order to form a belief on future messages, O2 needs a belief on the hypothesis and (since  O1 has perfect recall) a belief on all observations of O1 so far.  Clearly, the messages received till time \(k\) provide information about the observations of O1 till time \(k\) and are therefore included in the information state.


==> temp_test.tex <==
\input preamble
%\documentclass{IEEEtran}


\title {\LARGE \bf Decentralized Detection with Signaling}
%\author{Ashutosh Nayyar \hspace{8pt} Demosthenis Teneketzis}
\author{
Ashutosh Nayyar and Demosthenis Teneketzis 
\thanks{A.\ Nayyar and D.\ Teneketzis are with Department of Electrical Engineering and Computer Science,
        University of Michigan, Ann arbor. 
         {\tt\small anayyar@umich.edu, teneket@eecs.umich.edu}}
         }
\begin{document}
\maketitle
\begin{abstract}
    We consider a sequential problem in decentralized detection. Two observers can make repeated noisy observations of a binary hypothesis on the state of the environment. At any time, any of the two observers can stop and send a final message to the other observer or it may continue to take more measurements. After an observer has sent its final message, it stops operating.  The other observer is then faced 
with a different stopping problem. At each time instant, it can decide either to stop and declare a final decision
on the hypothesis or take another measurement. At each time, the system incurs an operating cost depending on the number of observers that are active at the time. A terminal cost that measures the accuracy of the final decision is incurred at the end. We show that, unlike in other sequential detection problems that do not involve communication between observers, two threshold rules on an observer's posterior belief no longer guarantee optimality in this problem. Thus the potential for signaling among observers alters the nature of optimal policies. We obtain a new parametric characterization of optimal policies for this problem.
\end{abstract}


\input Introduction

%\input problem_formulation

%\input information_states
%\input counterexample
%\input thresholds
%\input conclusion

%\input theorem1
%\input mtns_appendix
%\input mtns_appendix_part2
%\input appendix_2
%\input References
\end{document} 

==> theorem1.tex <==
\appendices


\section{Proof of Theorem 1 and Theorem 2}
 Consider an arbitrary choice \(\Gamma^2=(\gamma^2_1,\gamma^2_2,...,\gamma^2_{T2})\) for O2's policy. Note that for a fixed \(\Gamma^2\), \(\tau^2\) and \(U^2_{\tau^2}\) are functions of O2's observation sequence \((Y^2_1,Y^2_2,...,Y^2_{T^2})\) and messages received from O1 \((Z^1_1,...,Z^1_{T^1})\). In other words, a policy of O2 induces a stopping time function \(S^{\Gamma^2}\) and an estimate function \(R^{\Gamma^2}\) defined for all possible realizations of the observations of O2 and messages from O1 such that
\begin{equation}
   \tau^2 = S^{\Gamma^2}(Y^2_{1:T^2},Z^1_{1:T^1})
\end{equation}
\begin{equation}
      U^2_{\tau^2} = R^{\Gamma^2}(Y^2_{1:T^2},Z^1_{1:T^1})
\end{equation}
 \par
 A simple application of Bayes' rule shows that \(\pi^1_{k+1}\) can be updated from \(\pi^1_k\) and \(Y^1_{k+1}\).
 \begin{align}
   \pi^1_{k+1}= &P(H=0|Y^1_{1:k+1}) \nonumber \\
              = &\frac{P(Y^1_{k+1}|H=0)\pi^1_k}{P(Y^1_{k+1}|H=0)\pi^1_k+P(Y^1_{k+1}|H=1)(1-\pi^1_k)} \label{eq:Ap1}
 \end{align}
 Thus, we have that \[ \pi^1_{k+1} = T_k(\pi^1_k,Y^1_{k+1}), \] where \(T_k\) is defined by (\ref{eq:Ap1}).
 We will now use backward induction to show that the function \(V_k\) evaluated at \(\pi^1_k(y^1_{1:k})\) provides a lower bound for the expected cost to go function at time \(k\) under any policy for O1.
 \begin{align}
    V_{T^1}(\pi) := min\{&E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{T^1}=\pi,Z^1_{1:T^1-1}=b,Z^1_{T^1}=0], \nonumber \\
                         &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{T^1}=\pi,Z^1_{1:T^1-1}=b,Z^1_{T^1}=1] \}
 \end{align}
  
  
 For \(k=T^1-1,T^1-2,...,1\), we define,
 \begin{align}
  V_{k}(\pi) := min\{&E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{k}=\pi,Z^1_{1:k-1}=b,Z^1_{k}=0], \nonumber \\
                          &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{k}=\pi,Z^1_{1:k-1}=b,Z^1_{k}=0], \nonumber \\
                          &c^1 + E[V_{k+1}(T_k(\pi^1_k,Y^1_{k+1}))|\pi^1_{k}=\pi,Z^1_{1:k}=b]                               \}
 \end{align} 
 
We will show that the function \(V_k\) evaluated at \(\pi^1_k(y^1_{1:k})\) provides a lower bound for the expected cost to go function at time \(k\) under any policy for O1. We will employ the backward induction arguments of dynamic programming. First consider time \(T^1\). 
If observer 1 has not sent a final decision by time \(T^1\), then its expected cost to go at \(T^1\) is either
 \begin{equation}
   W_{T^1}(y^1_{1:T^1})=E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=0] \label{eq:Ap2} 
 \end{equation}
 if it sends a \(0\) at time \(T^1\) or
 \begin{equation}
               W_{T^1}(y^1_{1:T^1})=E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=1] \label{eq:Ap3}
 \end{equation}
 if it sends a \(1\) at time \(T^1\).
 Consider the expectation in (\ref{eq:Ap2}). We can write it as 
 \begin{align}
 	&E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=0] \nonumber \\
 	= &E^{\Gamma^2}[c^2S^{\Gamma^2}(Y^2_{1:T^2},Z^1_{1:T^1})+J(R^{\Gamma^2}(Y^2_{1:T^2},Z^1_{1:T^1}),H)|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=0] \nonumber\\
 	= &E^{\Gamma^2}[c^2S^{\Gamma^2}(Y^2_{1:T^2},b_{1:T^1-1},0)+J(R^{\Gamma^2}(Y^2_{1:T^2},b_{1:T^1-1},0),H)|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=0] \label{eq:Ap4}
\end{align}
 where we substituted \(Z^1_{1:T^1}\) in (\ref{eq:Ap4}) with the values specified in the conditioning term of the expectation. Since the only random variables left in the expectation in (\ref{eq:Ap4}) are \(Y^2_{1:T^2}\) and \(H\), we can write this expectation as
 \begin{align}
 	\sum\limits_{\{h=0,1\}} \sum\limits_{y^2_{1:T^2} \in \mathcal{Y}^{2}_{1:T^2}} [ P(y^2_{1:T^2},H=h|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=0)\{c^2S^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0)+J(R^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0),h)\}] \label{eq:Ap5}
 \end{align}
 Consider first the term for \(h=0\) in (\ref{eq:Ap5}). Because of the conditional independence of the observations at the two observers, we can write this term as follows:
 \begin{align}
   &\sum\limits_{y^2_{1:T^2} \in \mathcal{Y}^{2}_{1:T^2}} [P(y^2_{1:T^2}|H=0).P(H=0|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=0).\{c^2S^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0)+J(R^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0),0)\}] \nonumber \\
   =&\sum\limits_{y^2_{1:T^2} \in \mathcal{Y}^{2}_{1:T^2}} [P(y^2_{1:T^2}|H=0).\pi^1_{T^1}(y^1_{1:T^1}).\{c^2S^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0)+J(R^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0),0)\}] \label{eq:Ap5.1}
 \end{align}
 Similarly, the term for \(h=1\) in (\ref{eq:Ap5}) can be written as,
 \begin{equation} \label{eq:Ap6}
  \sum\limits_{y^2_{1:T^2} \in \mathcal{Y}^{2}_{1:T^2}} [P(y^2_{1:T^2}|H=1).(1-\pi^1_{T^1}(y^1_{1:T^1}))\{c^2S^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0)+J(R^{\Gamma^2}(y^2_{1:T^2},b_{1:T^1-1},0),1)\}]
 \end{equation}
 Combining equations (\ref{eq:Ap5.1}) and (\ref{eq:Ap6}), we see that the expectation in (\ref{eq:Ap5}) depends on \(\pi^1_{T^1}(y^1_{1:T^1})\) and not on the entire sequence \(y^1_{1:T^1}\). Hence, we can replace \(y^1_{1:T^1}\) by \(\pi^1_{T^1}(y^1_{1:T^1})\) in the conditioning. Therefore, in (\ref{eq:Ap2}), we  have 
 \begin{align}
 W_{T^1}(y^1_{1:T_1})= &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:T_1},Z^1_{1:T^1-1}=b,Z^1_{T^1}=0] \nonumber \\
   = &E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|\pi^1_{T^1}(y^1_{1:T_1}),Z^1_{1:T^1-1}=b,Z^1_{T^1}=0] \nonumber \\
   \geq &V_{T^1}(\pi^1_{T^1}(y^1_{1:T_1})) \label{eq:Ap7}
 \end{align}
 where we used the definition of \(V_{T^1}\) in (\ref{eq:Ap7}). Exactly same arguments hold when \(W_{T^1}(y^1_{1:T_1})\) is given by equation (\ref{eq:Ap3}). Hence, we conclude that the following inequality always holds:
 \[ W_{T^1}(y^1_{1:T_1}) \geq V_{T^1}(\pi^1_{T^1}(y^1_{1:T^1})) \]
 
 Now consider time \(k\). Assume that \[ W_{k+1}(y^1_{1:k+1}) \geq V_{k+1}(\pi^1_{k+1}(y^1_{1:k+1})) \] If observer 1 has not sent a final decision by time \(k\), then its expected cost to go at \(k\) is either
 \begin{equation} \label{eq:Ap7.1}
   W_{k}(y^1_{1:k})=E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:k},Z^1_{1:k-1}=b,Z^1_{k}=0] 
 \end{equation}
 or
 \begin{equation} \label{eq:Ap8}
               W_{k}(y^1_{1:k})=E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:k},Z^1_{1:k-1}=b,Z^1_{k}=1] 
 \end{equation}
 or
 \begin{equation}\label{eq:Ap9}
 	  W_{k}(y^1_{1:k})= c^1+ E^{\Gamma^2}[W_{k+1}(y^1_{1:k},Y^1_{k+1})|y^1_{1:k},Z^1_{1:k}=b]
 \end{equation}
 By arguments similar to those used at time \(T^1\), we can show that \(V_k\) is a lower bound to expressions in (\ref{eq:Ap7.1}) and (\ref{eq:Ap8}). That is,
 \begin{equation} \label{eq:Ap7.2}
   W_{k}(y^1_{1:k})=E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:k},Z^1_{1:k-1}=b,Z^1_{k}=0] \geq V_k(\pi^1_k(y^1_{1:k}))
 \end{equation}
and
 \begin{equation} \label{eq:Ap8.1}
               W_{k}(y^1_{1:k})=E^{\Gamma^2}[c^2\tau^2+J(U^2_{\tau^2},H)|y^1_{1:k},Z^1_{1:k-1}=b,Z^1_{k}=1] \geq V_k(\pi^1_k(y^1_{1:k}))
 \end{equation}
  Consider equation (\ref{eq:Ap9}). From the induction hypothesis at time \(k+1\), we have that
 \[ W_{k+1} (y^1_{1:k+1}) \geq V_{k+1}(\pi^1_{k+1}(y^1_{1:k+1})) \]
 which implies
 \begin{align}
 E^{\Gamma^2}[W_{k+1}(y^1_{1:k},Y^1_{k+1})|y^1_{1:k},Z^1_{1:k}=b]  \geq &E^{\Gamma^2}[V_{k+1}(\pi^1_{k+1}(y^1_{1:k},Y^1_{k+1}))|y^1_{1:k},Z^1_{1:k}=b] \nonumber \\
 = &E^{\Gamma^2}[V_{k+1}(T_k(\pi^1_k(y^1_{1:k}),Y^1_{k+1}))|y^1_{1:k},Z^1_{1:k}=b] \label{eq:Ap10}
 \end{align}
 The above expectation is a function of \(\pi^1_k(y^1_{1:k})\) the following conditional probability:
 \[ P(Y^1_{k+1}|y^1_{1:k},Z^1_{1:k}=b) \]
 which can be expressed as:
 \[P(Y^1_{k+1}|H=0).\pi^1_k(y^1_{1:k}) + P(Y^1_{k+1}|H=1).(1-\pi^1_k(y^1_{1:k})) \]
 
 Thus the expectation in (\ref{eq:Ap10}) depends only on \(\pi^1_k(y^1_{1:k})\) and not the entire sequence \(y^1_{1:k}\). Hence, it can be written as:
 \[E^{\Gamma^2}[V_{k+1}(T_k(\pi^1_k(y^1_{1:k}),Y^1_{k+1}))|\pi^1_k(y^1_{1:k}),Z^1_{1:k}=b]\] 
 Equation (\ref{eq:Ap10}) then implies that
 \begin{align}
 c^1+ E^{\Gamma^2}[W_{k+1}(y^1_{1:k},Y^1_{k+1})|y^1_{1:k},Z^1_{1:k}=b] \geq &c^1+ E^{\Gamma^2}[V_{k+1}(T_k(\pi^1_k(y^1_{1:k}),Y^1_{k+1}))|\pi^1_k(y^1_{1:k}),Z^1_{1:k}=b] \nonumber \\
 \geq &V_k(\pi^1_k(y^1_{1:k})) \label{eq:Ap11}
 \end{align}
 
 From equations (\ref{eq:Ap7.2}),(\ref{eq:Ap8.1}) and (\ref{eq:Ap11}), we can conclude that the inequality \(W_k(y^1_{1:k}) \geq V_k(\pi^1_k(y^1_{1:k}))\) always holds. Hence, by induction it holds for all \(k=T^1,T^1-1,...,2,1\). 
 \par
  A policy \(\gamma^{*}\) that always selects the minimizing option in the definition of \(V_k\) for each \(\pi\) will achieve the lower bounds \(V_k\) on \(W_k\) with equality for all \(k\).  Note that the total cost of a policy for O1 is \(E[W_1(y^1_1)]\) which must be greater that \(E[V_1(\pi^1_1(y^1_{1}))]\). Thus, we have that \(\gamma^{*}\) achieves the lower bound on total cost for any policy. Hence, it is  optimal. Thus, an optimal policy is given by selecting the minimizing option in definition of \(V_k\) at each \(\pi\). In other words, there is an optimal policy of the form:
 \[Z^1_t = \gamma^{*}_{t}(\pi^{1}_{t})\]
